Data-Driven Constitutive Relation Reveals Scaling Law for Hydrodynamic Transport Coefficients

Finding extended hydrodynamics equations valid from the dense gas region to the rarefied gas region remains a great challenge. The key to success is to obtain accurate constitutive relations for stress and heat flux. Data-driven models offer a new phenomenological approach to learning constitutive relations from data. Such models enable complex constitutive relations that extend Newton's law of viscosity and Fourier's law of heat conduction by regression on higher derivatives. However, the choices of derivatives in these models are ad-hoc without a clear physical explanation. We investigated data-driven models theoretically on a linear system. We argue that these models are equivalent to non-linear length scale scaling laws of transport coefficients. The equivalence to scaling laws justified the physical plausibility and revealed the limitation of data-driven models. Our argument also points out that modeling the scaling law could avoid practical difficulties in data-driven models like derivative estimation and variable selection on noisy data. We further proposed a constitutive relation model based on scaling law and tested it on the calculation of Rayleigh scattering spectra. The result shows our data-driven model has a clear advantage over the Chapman-Enskog expansion and moment methods.

==> deleted.tex <==
\begin{equation} \label{The Linear Model on Derivatives: stress_and_flux, not flux, Fourier1}
	\begin{split}
		  M(\Kn) &= \frac{4}{3} \frac{\mu(\Kn)}{ \mu_0} \\
K(\Kn)&=\frac{\kappa(\Kn)}{\kappa_0},
	\end{split}
\end{equation}

non-dimensional scaling functions in which we replace $k$ in \eqref{The Linear Model on Derivatives: stress_and_flux, not flux, Fourier} with $\Kn$ because they are equivalent for even functions. The real functions $M$ and $K$ are modeled and computed in our study via neural networks from data. 

We argued that linear regression for constitutive relations as \eqref{The Linear Model on Derivatives: stress_and_flux general} is equivalent of modeling scaling functions $\mu(k), \kappa(k)$ in \eqref{The Linear Model on Derivatives: stress_and_flux, not flux, Fourier}. The test its viability, we model the scaling functions with constraint neural network and test them on calculating the density fluctuation spectra.

Particularly, we are interested in changes from coarse-scale ($k=0$) to fine-scale ($k>0$), which is the inverse of the usual fine-scale to coarse-scale renormalization group theory. Therefore the scaling functions $\mu(k), \kappa(k)$ describe an inverse scaling law of transport coefficients.

The reason that macroscopic models are inaccurate is they lacks accurate constitution relation for the unclosed terms, i.e the shear stress $\sigma$ and heat flux $q$. They could be modeled as functional of velocity and temperature field, such as the Navier-Stokes(NS) equation\cite{Landau1987} and Burnnet\cite{Burnett1936,chapman1990mathematical} equations, or as additional equations by taking higher moments of the Boltzmann equation under the assumption of Maxwell molecules\cite{maxwell1867iv}, which gives the Grad 13 equations\cite{Grad1949}. These constitution relation are valid at small knudsen number, but fails when the Knudsen number of the system is large, because they are either perturbation result at small Knudsen number, or expansion near equilibrium with slow convergence. For high Knudsen number, more flexible constitution relation model with better asymptotic behavior is expected. However, such constitution relation is in general hard to derive without techniques such as perturbation or expansion.

However, these application is still limited to system with known governing equation or artificially designed simple cases. For attempts to learn PDE, the major difficulties of is to select and estimate high order derivatives. As for constructing the distribution $f$, the difficulty is to ensure consistency with known thermodynamic quantities. Other obstacles for both approach is how to make the system stable by respect the second law of thermodynamics, and how to model the change of the system as Knudsen number changes.

In this letter, we proposed a linear constitution relation (LCR) model and applied this model to calculate the Rayleigh scattering spectra. We unified the two approach: learning a PDE and construct distribution $f$, and analyzed the underlying assumption of the unification. We bypassed the difficulty on estimation and selection of high order derivatives through Fourier analysis. We ensured the stability of our linear constitution relation model by making the entropy non-decreasing. We also modeled the change of the system as Knudsen number changes. Our linear constitution relation model performs much better than Chapman Enskog expansion and Grad moment method.

, especially in the transition region of length scales from dense gas scale to rarefied gas scale


\paragraph{Methods} The system we considered is the Rayleigh Scattering under the fluctuation of a homogeneous simple gas. The Rayleigh scattering is caused by scattering of electromagnetic wave (EM wave) due to the thermodynamic density fluctuation of gas, which affect the dielectric constant hence the refraction index\cite{jackson1999classical,landau2013classical}. The interaction between EM wave and density fluctuation wave from collective gas molecule behavior, will change the frequency of scattered EM wave. The intensity of scattered EM wave $I$ at each frequency is the Rayleigh scattering spectra, and is proportional to the density fluctuation spectra of gas\cite{Pecora1964,Kilmister1989}. The density fluctuation spectra is the Fourier transformation of density correlation function, and is proportional to the amplitude of the density fluctuation at each wave length and frequency,
\begin{equation} \label{Rayleigh Scattering Spectra: spectral density for with space-time correlation function, omega4}	
\begin{split}
	\mathbf{I}(\omega_f) &\propto \omega_i^4 \left<\rho^2\right>(\mathbf{k},\omega) \\
	\mathbf{k}&= \mathbf{k}_i-\mathbf{k}_f \\
	\omega&= \omega_i-\omega_f \\
	\left| \mathbf{k}_{i,f}\right|&=\frac{\sqrt{\epsilon_{0}} \omega_{i,f}}{c}\\
\end{split}
\end{equation}
where $\mathbf{k}$ represents the wave vector, $\omega$ is the angular frequency, and the subscript $i$ and $f$ represents incident and scattered EM wave, $\epsilon_{0}$ is the dielectric constant of gas, $c$ is the speed of light, and the direction of $\mathbf{\hat{k}}_{f}$ is the direction pointing from the scattering center to the observer. To calculate the Rayleigh spectra we need to accurately compute the density fluctuation spectra $\left<\rho^2\right>(\mathbf{k},\omega)$. 

Now we introduce the governing equation of the system. The 1D non-dimensionalized and linearized conservation law for a small perturbation of mass, momentum and energy is 

for which the non-dimensionalization is discussed in supplimentary material. The density spectra $\left<\tilde{\rho}^2\right>(k)$, could be obtained by multiply the equation with $\tilde{\rho}(0,0)$ at time $0$ and position $0$, then taking Fourier transform after the ensemble average. The unclosed terms are the stress $\sigma$ and heat flux $q$. To close the equation, the most obvious approach is to formulate them as functional of other macroscopic quantities.

To calculate the density fluctuation spectra, we need the macroscopic governing equation for the flow system and analysis the thermodynamic fluctuation accordingly. The system could be completely described by the linearized Boltzmann equation \cite{Yip1964}. Therefore only linearized macroscopic equation need to be considered. Meanwhile, given the observation direction, the thermodynamic velocity fluctuation of in fluid could be decomposed into transverse and longitudinal part \cite{Landau1980}, and only longitudinal fluctuation contributes to density fluctuation, hence the problem could be reduced to a 1D problem.

To reformulate the problem, certain physical observations and constraints should be considered. We wish the Knudsen number completely determine the system, however, the coefficient $a_n, b_n$ will introduce additional non-dimensional to the system. Therefore these coefficients must be function of the Knudsen number $\mbox{Kn}$. It is more convenient to analysis the series in Fourier space since the Knudsen number in this problem is related to the wave number. The linear combination of derivatives in Eq \ref{The Linear Model on Derivatives: stress_and_flux} is a sum of a polynomial series of $k$ in Fourier space, hence it is also function of $\mbox{Kn}$. Under the constraint that the entropy is non-decreasing, we could reformulate the previous model Eq \eqref{The Linear Model on Derivatives: stress_and_flux} as the linear constitutive relation model in Fourier space:
\begin{equation} \label{The Linear Model on Derivatives: stress_and_flux, not flux, Fourier}
	\begin{split}
		 \tilde{\sigma}_{xx}(k) & = -i k A(Kn)\tilde{v}_k; \quad A(Kn) \ge 0 \\
		\tilde{q}_{x}(k) &=-i k B(Kn)\tilde{T}_k; \quad B(Kn) \ge 0   \\
	\end{split}
\end{equation}
where the function $A(\mbox{Kn})$ and $B(\mbox{Kn})$ are non-negative real function of the Knudsen number $\mbox{Kn}$, and they are not necessarily to be linear. Note that the multiplication in Fourier space is equivalent to a convolution, Eq \eqref{The Linear Model on Derivatives: stress_and_flux, not flux, Fourier} is equivalent to a convolution in real space. In this formulation, we converted the problem of learning an infinite discrete set of coefficient $a_n, b_n$, to a function learning problem on $A,B$, which is much easier to do. In practice, we model the function $A,B$ as neural network, the flow chart Fig \ref{fig:Flowchart} represents how to utilize the constitutive relation model. 

In another view, the function $A,B$ could be treated as function of adaptive viscosity $\mu(\mbox{Kn})$ and heat conduction coefficient $\kappa(\mbox{Kn})$ for different Knudsen number

where $\mu_0$ is the viscosity coefficient for NS equation. In this view, another non-dimensional number, the Prandtl number, that defined as the ratio of momentum diffusivity to thermal diffusivity, appears. The Hilbert Chapman Enskog theory tell us a constant Prandtl number $\frac{2}{3}$ for monotomic gas\cite{Kilmister1989}. We could set the Prandtl number to be $\frac{2}{3}$ by requiring
\begin{equation} \label{Fix Pr}
A(\mbox{Kn}) = \frac{16}{45}B(\mbox{Kn})
\end{equation}
and in practice this additional constraint will not affect the performance of our linear constitutive relation model. This indicates that the Prandtl number do not change much as the Knudsen number changes in our case. Another thing worth noting is that the NS equation also lies in this framework, we have
\begin{equation} \label{NS,A}
A_{NS}(\mbox{Kn}) = \frac{4}{3}\mbox{Kn}
\end{equation}

To determine the unknown coefficients $\mathbf{W}_{1,2}$, we have to define a loss function to be minimized during training process. For a reasonable initialization of $\mathbf{W}_{1,2}$, we could compute the predicted density fluctuation spectra $\left<\rho^2\right>_{LCR} (k,\omega;\mathbf{W}_{1,2})$ using the governing equation Eq and the constitutive relation. This predicted density fluctuation spectra is the compared with the spectra calculated numerically with DSMC method. We define the loss function that measures the difference between the spectra predicted by linear constitutive relation model and the DSMC method as

in which the expectation $\mathbb{E}_{k \sim U}$ is taken numerically by sampling $k$ uniformly from the desired range of $k$, which corresponds to our desired range of Knudsen number, and the expectation $ \mathbb{E}_{\omega \sim p(\omega|k)}$ is sampled from from the distribution $p(\omega|k)$ that is proportional to the amplitude of the DSMC spectra 
\begin{equation} \label{The omega distribution}
    p(\omega|k) \propto  \left<\rho^2\right>_{DSMC} (k,\omega)
\end{equation}
which makes the sample point lies more on the region we interested such as peaks. 

The unknown coefficients $\mathbf{W}_{1,2}$ is therefore determined by the optimization process
\begin{equation} \label{The loss function}
    \mathbf{W}_{1,2} = \mathop{\arg\min}\limits_{\mathbf{W}_{1,2}} L(\mathbf{W}_{1,2})
\end{equation}
which is a non-convex optimization problem whose optimal solution is in general hard to find. However, stochastic optimization process could help us to get a nice solution. In our case, we use the ADAM \cite{Kingma2015} optimizer to solved by the optimization problem. 

\begin{equation} \label{The omega, no dim}
\tilde{\omega} = \frac{\omega}{c k}
\end{equation} 

The spectra $\left<\delta \tilde{\rho}^2\right>(\tilde{\omega})$ for given Knudsen number are shown in Fig \ref{spectra}, with comparesion among DSMC, NS equation, Grad 13 method and our LCR model. The frequency $\tilde{\omega}$ is the non-dimensionalized frequency, in which $c$ is the speed of sound and $k$ is the wavenumber we are considering. When the Knudsen number is small, the interaction between gas molecules give the major contribution to the density fluctuation spectra. Three peak appears, with the middle one due to the entropy fluctuation process which corresponds to the heat diffusion, and the two peak on each side are caused by pressure fluctuation corresponding to sound wave propagation. It is evident that all model are consistent under small Knudsen number. However, as the Knudsen number increases, the interaction between gas molecules are weaken, while Maxwellian diffusion gives more contribution. The structure of the spectra therefore disappear gradually, blur into a bell shape. The shape and amplitude of NS and Grad 13 method deviate from DSMC result at large Knudsen number, while the linear constitutive relation model still gives correct spectra. It is known\cite{Wu2020} that higher order Chapman Enskog expansion will not increase the accuracy of spectra, and huge amount of moment is needed to increase the accuracy of Grad moment method. Since we only used three moments, the advantage using data-driven approach is obvious.

The learnt result of the function $A$ is shown in Fig \ref{fig:AKn}. Instead of a straight line, our LCR model result shows a decrease from NS equation as the knudsen number increase. This means the viscosity coefficient decrease as the Knudsen numeber increase. This is reasonable since as Knudsen number increase, the collision frequency between gas particle decrease hence weaken the viscosity. 

One may concern about the generalization ability of the linear constitutive relation model, because the performance on the density spectra may merely because we trained the model on the density spectra. We test the LCR model performance on predicting the velocity spectra, result is shown in Fig \ref{velocity}. The performance is still much better than NS equation. This shows that our LCR model, though learnt from the density fluctuation spectra, have the generalization power to predict spectra of other quantities.

In summary, we have proposed an easy to learn data driven linear constitutive relation model with physical concerns such as entropy change. We have discussed the underlying assumption for our model, showed that the freedom we have to model stress and heat flux using arbitrary model comes with a price that we are limited to near equilibrium case. We applied the linear constitutive relation model to predict the Rayleigh scattering spectra, which is equivalent to predict the density fluctuation spectra of gas, and shown it performs better that traditional Chapman Enskog derived NS equation and Grad 13 moment equation. The generalization ability of the linear constitutive relation is also shown through predicting the velocity fluctuation spectra.

Now we propose a form of the functional in order to model the functional $\sigma$ and $q$ on other macroscopic quantities. An essential physics constraint that ensure the stability of the system is the entropy change of the gas. The change rate of entropy $s$ for the gas \cite{Landau1987} is given as follows, 

 which should be is non-negative. To make the entropy to be non-decreasing, we require that $q$ to be a functional of $T$ only, and $\sigma$ to be a functional of $v$. The reason is they fluctuate independently according to fluctuation theory \cite{Landau1980}, hence to ensure that both terms in Eq \ref{Hydrodynamic Fluctuations:Total entropy change rate, expand 1} are non-negative, we need to treat them separately. Because the system we considering is linear, we assume that the functional takes the form:

where $a_n, b_n$ are undetermined coefficients. However, these undetermined coefficients are infinite and discrete. It is hard to determine which coefficient is non-zero, even with the sparsity coefficient estimation technique such as L1 regularization \cite{tibshirani1996regression,friedman2001elements}. Another difficulty is the estimation of high order derivatives, which will introduce large numerical error into the system as the order becomes higher and higher\cite{Raissi2019}. To overcome these difficulty, a certain reformulation of the problem to make the undetermined coefficients easy to learn is required.


We discuss the underlying assumption before we model the unclosed terms. Actually, the freedom we have to model stress and heat flux without constraints comes with a price that we are limited to near equilibrium case. It is well known that $\sigma$ and $q$ are moments of the one particle distribution $f(x,\mathbf{u}, t)$ governed by the Boltzman equation. The molecule velocity $\mathbf{u}$ is the possible velocity of a particular gas molecule, and should be distinguished with the macroscopic velocity of a gas parcel $\mathbf{v}$. We could construct the distribution analogous to the Hilbert expansion used in Grad moment method that allow us to have arbitrary $\sigma$ and $q$:

where $\mathbf{c} = \mathbf{u} - \mathbf{v}$ is the peculiar velocity. We used the Einstein summention convention in this equation. In this construction of $f$, all terms in the construction are fixed except the stress $\sigma$ and heat flux $q$ tensor, give us the theoretical support to model them as arbitrary functional of other macroscopic quantities such as $v$ and $T$. We claim that attempts to learn a PDE by substitute $\sigma$ and $q$ with functional of other quantities \textbf{without} constraints, implicitly use the assumption that the distribution $f$ could be described by expansion in equation \ref{f}. It is valid in our case since we are considering fluctuation near equilibrium. However, for strong non-equilibrium case, this assumption will expected to fail, therefore proper constraints must be imposed to model strong non-equilibrium cases.

\begin{equation}\label{f}
	\begin{split}
f &= f_0(1+h)\\
f_0 &= \frac{\rho}{m(2\pi k_b T/m )^{3/2}} \exp(-\frac{m\mathbf{c}^2}{2k_B T} ) \\
		h &= \frac{3}{4}\mbox{Kn} (\tilde{c}_i \tilde{c}_j -\frac{1}{3}\delta_{ij}\mathbf{\tilde{c}}^2)\tilde{\sigma}_{ij}  +\frac{\mbox{Kn}}{\mbox{Pr}} (\frac{\tilde{\mathbf{c}}^2}{2}-\frac{5}{2})\tilde{c}_i  \tilde{q}_{i}\\
	\end{split}
\end{equation}


Another possible issue for the inference of function A is the uncertainty introduced through data-driven process. Data-driven is essentially accompanied with Monte-Carlo sampling error, or say, the uncertainty. In our case, different run of training process may leads to slightly different function A. However, this difference is small and will not change the general shape of the graph of function A. To address this issue, further research on uncertainty quanlification technique or Bayesian inference may be applied to give an quantitative description of this uncertainty.

The Rayleigh scattering, having discovered by Lord Rayleigh back to the nineteenth-century, was the the reason for the blue color of the sky at daytime and twilight. The spectra shape of the Rayleigh scattering depends on the incident light wavelength. If the mean free path of the gas is much greater than the wavelength of the incident light, then we say that the scattering occurs in \textbf {Knudsen regime}. In this case, the Rayleigh scattering spectrum is approximately Gaussian, because the gas molecules lacks interaction and does not have collective effects. If the mean free path of the gas is much smaller than the wavelength of the incident light (dense gas or liquid), then we call it \textbf{hydrodynamic regime}. The spectrum has the peaks corresponding to the sound wave of the gas. If the mean free path of the scattering gas medium is equivalent to the wavelength of the incident light, we call it \textbf{kinetic regime}, and the spectra is a complex mixture of Knudsen spectrum and hydrodynamic spectrum.

An effective way to model accurate constitutive relations will replace mesoscopic simulation, reduce the computational cost of flow simulation, hence boost industrial aerospace engineering.

We consider the constitutive relation for the stress and the heat flux as functionals. These functionals should be linear because the macroscopic governing equations are linear. It is natural to model these functionals as spatial derivatives of macroscopic quantities, linearly combined by coefficients, with the spatial derivatives and the coefficients for linear combinations estimated from observed data. However, noisy data causes difficulties in both derivative calculation \cite{Raissi2019} and coefficient estimation\cite{tibshirani1996regression,friedman2001elements?}. To bypass these difficulties, we propose the DUAL model for constitutive relation functionals. The functionals in the DUAL model are multiplications in the Fourier space, between macroscopic quantities and real functions $M({k})$ and $K({k})$,

To calculate the density fluctuation spectra, we analyze the thermodynamic fluctuation according to macroscopic governing equations. These macroscopic governing equations are linear because we know that the linearized Boltzmann equation could completely describe the Rayleigh scattering problem\cite{Yip1964}. In addition, these macroscopic governing equations have one dimension in spatial coordinates because only longitudinal density fluctuation contributes to Rayleigh scattering\cite{Landau1980, ?}. Therefore, the macroscopic governing equations form a 1D linear PDE system. Its non-dimensionalized version is defined as follows,

The next step should be learning the weights vector of the neural network $\mathbf{W}_{1,2}$. Learning the unknown coefficients $\mathbf{W}_{1,2}$ from data requires a loss function as the learning target. In our case, the loss function compares the difference between the observed and predicted spectra. The former are results from the DSMC method, while the latter are the predictions of the governing equation and the constitutive relation. We define the loss function as follows,

\begin{figure}
\includegraphics[width=2in]{FunctionAinpaper.PNG}% Here is how to import EPS art
\caption{\label{fig:AKn} The function $Kn M(Kn)$ inferred from DSMC data by the DUAL model, compared with the corresponding function for the NS equation. }
\end{figure}
\paragraph{Discussion} 

We consider the constitutive relation for the stress and the heat flux as functionals. These functionals should be linear because the macroscopic governing equations are linear. We assume constitutive relation functionals has the following form:

where $\tilde{M}, \tilde{K}$ are convolution kernel. We propose the DUAL model for constitutive relation functionals. The functionals in the DUAL model are multiplications in the Fourier space, between macroscopic quantities and real functions $M({k})$ and $K({k})$, 

They are functions of the non-dimensionalized wavenumber $k$, hence are also functions of the Knudsen number, as Eq \eqref{Kn} shows. 
